Optimization-Based Deep learning methods for Magnetic Resonance Imaging Reconstruction and Synthesis

This dissertation is devoted to provide advanced nonconvex nonsmooth variational models of (Magnetic Resonance Image) MRI reconstruction, efficient learnable image reconstruction algorithms and parameter training algorithms that improve the accuracy and robustness of the optimization-based deep learning methods for compressed sensing MRI reconstruction and synthesis. The first part introduces a novel optimization based deep neural network whose architecture is inspired by proximal gradient descent for solving a variational model. The second part is a substantial extension of the preliminary work in the first part by solving the calibration-free fast pMRI reconstruction problem in a discrete-time optimal control framework. The third part aims at developing a generalizable Magnetic Resonance Imaging (MRI) reconstruction method in the meta-learning framework. The last part aims to synthesize target modality of MRI by using partially scanned k-space data from source modalities instead of fully scanned data that is used in the state-of-the-art multimodal synthesis.

==> bibliography.tex <==
% This setup has you inputting the bibliography manually, this can be done away with by using
% BiBTeX, but that has not been used/implemented in this template, so, you are free/encouraged
% to use it to make your life much easier, but we are still in the process of integrating BiBTeX
\begin{thebibliography}{100}
\pagestyle{plain}
\bibitem{book:guide}
The~Editorial Office of the Graduate School,
\newblock \emph{Guide for Preparing Theses and Dissertations},
\newblock The University of Florida, \emph{Revised} 1998.

\bibitem{abdulra.m.sheikh.auh.ea:94}
M.~Abdulrahan, A.~U.~H. Sheikh, and D.~D. Falconer,
\newblock ``Decision feedback equalization for {CDMA} in indoor wireless
  communications,''
\newblock \emph{IEEE Journal on Selected Areas in Communications}, vol. 12, no.
  4, pp. 698--706, May 1994.

\bibitem{barbosa.an.miller.sl:98}
A.~N. Barbosa and S.~L. Miller,
\newblock ``Adaptive detection of {DS/CDMA} signals in fading channels,''
\newblock \emph{IEEE Transactions on Communications}, vol. 46, no. 1, pp.
  115--124, Jan. 1998.

\bibitem{barghou.rt.stuber.gl:92}
R.~T. Barghouthi and G.~L. St{\"u}ber,
\newblock ``Sequence acquisition techniques for {CDMA} systems employing
  {Kasami} sequences,''
\newblock in \emph{Proceedings~IEEE Military Communications Conference}, San
  Diego, CA, 1992, vol.~2, pp. 633--637.

\bibitem{barghou.rt.stuber.gl:94}
R.~T. Barghouthi and G.~L. St{\"u}ber,
\newblock ``Rapid sequence acquisition for {DS/CDMA} systems employing {Kasami}
  sequences,''
\newblock \emph{IEEE Transactions on Communications}, vol. 42, no. 2/3/4, pp.
  1957--1968, Feb./Mar./Apr. 1994.

\bibitem{bensley.se.aazhang.b:96}
S.~E. Bensley and B.~Aazhang,
\newblock ``Subspace-based channel estimation for code division multiple access
  communication systems,''
\newblock \emph{IEEE Transactions on Communications}, vol. 44, no. 8, pp.
  1009--1020, Aug. 1996.

\bibitem{bensley.se.aazhang.b:98}
S.~E. Bensley and B.~Aazhang,
\newblock ``{Maximum}-{Likelihood} synchronization of a single user for
  code-division multiple-access communication systems,''
\newblock \emph{IEEE Transactions on Communications}, vol. 46, no. 3, pp.
  392--399, Mar. 1998.

\bibitem{bershad.nj.qu.lz:89}
N.~J. Bershad and L.~Z. Qu,
\newblock ``On the probability density function of the {LMS} adaptive filter
  weights,''
\newblock \emph{IEEE Transactions on Acoustics, Speech and Signal Processing},
  vol. 37, no. 1, pp. 43--56, Jan. 1989.

\bibitem{braun.wr:97}
W.~R. Braun,
\newblock ``{PN} acquisition and tracking performance in {DS/CDMA} systems with
  symbol-length spreading sequences,''
\newblock \emph{IEEE Transactions on Communications}, vol. 45, no. 12, pp.
  1595--1601, Dec. 1997.

\bibitem{buehrer.rm.kaul.a.ea:96}
R.~M. Buehrer, A.~Kaul, S.~Striglis, and B.~D. Woerner,
\newblock ``Analysis of {DS-CDMA} parallel interference cancellation with phase
  and timing errors,''
\newblock \emph{IEEE Journal on Selected Areas in Communications}, vol. 14, no.
  8, pp. 1522--1535, Oct. 1996.

\bibitem{buehrer.rm.woerner.bd:95}
R.~M. Buehrer and B.~D. Woerner,
\newblock ``Analysis of adaptive multistage interference cancellation for
  {CDMA} using an improved {Gaussian} approximation,''
\newblock in \emph{Proceedings~IEEE Military Communications Conference}, San
  Diego, CA, 1995, vol.~3, pp. 1195--1199.

\bibitem{chang.rw.sriniva.r:80}
R.~W. Chang and R.~Srinivasagopalan,
\newblock ``Carrier recovery for data communication systems with adaptive
  equalization,''
\newblock \emph{IEEE Transactions on Communications}, vol. COM--28, no. 8, pp.
  1142--1153, Aug. 1980.

\bibitem{clarke.rh:68}
R.~H. Clarke,
\newblock ``A statistical theory of mobile-radio reception,''
\newblock \emph{The Bell System Technical Journal}, vol. 47, no. 6, pp.
  957--1000, July-Aug. 1968.

\bibitem{couch-ii.lw:97}
L.~W. Couch~II,
\newblock \emph{Digital and Analog Communication Systems},
\newblock Prentice-Hall, 5th edition, 1997.

\bibitem{davies.rb:73}
R.~B. Davies,
\newblock ``Numerical inversion of a characteristic function,''
\newblock \emph{Biometrika}, vol. 60, no. 2, pp. 415--417, 1973.

\bibitem{davies.rb:80}
R.~B. Davies,
\newblock ``The distribution of a linear combination of $\chi^2$ random
  variables,''
\newblock \emph{Applied Statistics}, vol. 29, no. 3, pp. 323--333, 1980.

\bibitem{douglas.sc.meng.thy:92}
S.~C. Douglas and T.~H.-Y. Meng,
\newblock ``Exact expectation analysis of the {LMS} adaptive filter without the
  independence assumption,''
\newblock in \emph{Proceedings~IEEE International Conference on Acoustics,
  Speech and Signal Processing}, San Francisco, CA, 1992, vol.~4, pp. 61--64.

\bibitem{douglas.sc:93}
S.~C. Douglas,
\newblock ``Exact expectation analysis of the {LMS} adaptive filter for
  correlated {Gaussian} input data,''
\newblock in \emph{Proceedings~IEEE International Conference on Acoustics,
  Speech and Signal Processing}, Minneapolis, MN, 1993, vol.~3, pp. 519--522.

\end{thebibliography}


==> tex/abbreviations.tex <==
%%-----------List of Symbols, Nomenclature or Abbreviation--------

%% Please note: a list of Symbols, terms, acronyms, etc. is not usually the best practice.
%% More often you should simply define an abbreviation the first time it is used.
%% If you DO need to include a list like this please notice that it must be paginated manually
%% by breaking it up into page size tables. Longtable will not wrap the definition properly if
%% it extends to a second line and a similar issue is encountered when the tabbing environment
%% is used. If you have a better way of meeting the Editorial Office requirements I'd love to hear about it.

\chapter*{LIST OF SYMBOLS, NOMENCLATURE, OR ABBREVIATIONS} \addcontentsline{toc}{chapter}{LIST OF SYMBOLS} %Start
%writing here. This is optional.
\singlespacing
\begin{tabular}{l p{5in}} %if the terms in the first column are longer than 1.4 inches reduce the number 5 appropriately
$\sum$ & Denotes the summation of a series of terms\\
\\%This adds the single space between definitions (required)
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\

\end{tabular}

\begin{tabular}{lp{5in}}
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
\end{tabular}
\doublespacing


